Online Policy Learning from Offline Preferences

In preference-based reinforcement learning (PbRL), a reward function is learned from a type of human feedback called preference. To expedite preference collection, recent works have leveraged \emph{offline preferences}, which are preferences collected for some offline data. In this scenario, the learned reward function is fitted on the offline data. If a learning agent exhibits behaviors that do not overlap with the offline data, the learned reward function may encounter generalizability issues. To address this problem, the present study introduces a framework that consolidates offline preferences and \emph{virtual preferences} for PbRL, which are comparisons between the agent's behaviors and the offline data. Critically, the reward function can track the agent's behaviors using the virtual preferences, thereby offering well-aligned guidance to the agent. Through experiments on continuous control tasks, this study demonstrates the effectiveness of incorporating the virtual preferences in PbRL.

==> pb_ail_contents/data_creation.tex <==
\subsection{Tasks}

\subsubsection{Ant}
This is a representative control task with low-dimensional states and actions available in the Gymnasium library\footnote{\url{https://github.com/Farama-Foundation/Gymnasium}}, and detailed description is available at its website. The agent needs to control an ant robot to move to the right as fast as possible without falling over. The agent is positively rewarded if its actions speedup the robot, and it is negatively rewarded by the magnitude of control forces and contact forces. The agent observes 27-dimensional vectors containing quantities such as the coordinates and velocities of the ant's torso. To control the ant, the agent needs to coordinate the four legs by controlling torques applied to the joints of its legs, a eight-dimensional vector.

This is an example for scenarios where what humans can perceive differs from the agent's state. Humans examine the learned behaviors by watching videos rendered from states.~\Cref{fig:ant_demo} shows an example for rendered states. While it is possible to tell if the ant is moving from videos, it is difficult if not impossible to determine some parts of states. For example, as the two legs at the remote end are partially blocked by the torso, it is impossible to observe the angles between these legs and the torso. Moreover, the agent observes all quantities used in calculating its rewards, but humans cannot observe control forces and contract forces.

\subsubsection{Humanoid}
This is a representative control task with low-dimensional actions but high-dimensional states available in the Gymnasium library. The agent needs to control a bipedal robot to move to the right as fast as possible without falling over. States are 376-dimensional vectors containing the coordinates, velocities, orientations of the robot and angles and angular velocities between parts of the robot. Actions are 17-dimensional vectors containing torques applied to joints of the parts of the robot. 

Besides the perception difference of Ant, this task is also an example for scenarios where humans observe irrelevant information that might mislead their assessments. An image for a rendered state is shown in~\cref{fig:humanoid_demo}. The multiple parts of the robot's body, torso, abdomen, and pelvis, can shake or remain stable while the robot is moving right. From a human's perspective, this means it can demonstrate different walking styles, or levels of proficiency. Yet differences in styles or proficiency do not necessarily relate to difference in sums of groundtruth reward. 

\subsubsection{HumanoidStandup}
This task is a variant of Humanoid. It uses the same bipedal robot, state specification and action specification as in Humanoid. Unlike Humanoid, this task starts with the robot laying on the ground, and the agent is requires to control the robot to stand up.~\Cref{fig:humanoid_standup_demo} provides an example for an initial state of this task.

HumanoidStandup differs from Ant and Humanoid in that decisions are awarded for how much the robot has moved upward (the value of its z-coordinate), while in the other two tasks decisions are awarded for speed difference they caused. This means that it is easier for humans to compare videos for different trajectories for HumanoidStandup, as they can evaluate achievements for moving upward by the extent parts of the robot are perpendicular the the ground. Meanwhile, for Ant and Humanoid, it is difficult to tell the speed difference as robots do not appear in the same video. Nevertheless, humans still not able to observe contact forces or control forces that are also parts of the rewards.



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{cdpl_contents/figures/ant.jpeg}
         \caption{Ant}
         \label{fig:ant_demo}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{cdpl_contents/figures/humanoid.jpeg}
         \caption{Humanoid}
         \label{fig:humanoid_demo}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{cdpl_contents/figures/humanoid_standup.jpeg}
         \caption{HumanoidStandup}
         \label{fig:humanoid_standup_demo}
     \end{subfigure}
\end{figure}

\subsection{Trajectory Generation}
For Ant, Humanoid and HumanoidStandup, trajectories are generated by soft actor-critic (SAC)~\citep{Haarnoja2018} agents which are trained from scratch using the implementation provided by~\citet{NEURIPS2021_670e8a43}. This study uses the hyperparameter values reported in~\Cref{tab:expert_hyper} to train five agents for each task.~\Cref{tab:expert_final} shows the final performance of each agent and the average performance for each task.

As the goal is to collect trajectories from two policies of different optimality, for each agent we first select two checkpoints based on some performance thresholds. The threshold for "bad" policy is determined as 0.3 times the average final performance of this task, and the threshold for "good" policy is 0.7 times the average final performance. For Ant, Humanoid, and HumanoidStandup, the former threshold values are 1396.8, 1396.8, 31423.6, respectively. The latter threshold values are 4888.8, 4888.8, and 109982.5, respectively. In total, for each task 20 policies are used in trajectory generation. 

With each policies, we generate 200 trajectories. For Ant, Humanoid, and HumanoidStandup, trajectories terminate if a terminating signal is received from the environment, or if the number of steps exceed 1000. Then, we select the first ten trajectories generated by every policy as the ones to be annotated and aggregate them into a set of 100 trajectories to be annotated. 

\begin{table}[t]
\caption{Hyperparameters for the SAC learner.}
\label{tab:expert_hyper}
\centering
\scriptsize
\begin{tabular}{ll}
\toprule
Parameter &Value \\ \midrule
optimizer                                & Adam \\
learning rate for the actor              & $3\times10^{-4}$ \\
learning rate for the critic             & $3\times10^{-4}$ \\
whether to train alpha                   & Yes \\
initial value for alpha                  & 0.1 \\
learning rate for alpha                  & $3\times10^{-4}$ \\
\#hidden layers (all networks)                  & 2 \\
\#units per layer for the actor          & 256 \\
\#units per layer for the critic         & 256 \\
\# training steps                        & 1 \\
\# environment steps per training step   & 1\\
activation function (all networks)       & ReLU \\
interval for updating the target network & 1\\
smoothing coefficient for target updates & $5\times10^{-3}$ \\
size of replay buffer                    & $1\times10^6$ \\
discount factor                          & 0.99 \\\bottomrule
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Final performance of agents trained to generate trajectories for Ant, Humanoid, and HumanoidStandup.}
\label{tab:expert_final}
\centering
\scriptsize
\begin{tabular}{lllllll}
\toprule
Task               & Agent 1  & Agent 2  & Agent 3  & Agent 4  & Agent 5  & Avg. \\\midrule
Ant-v4             & 7397.9   & 7334.2   & 6093.2   & 7418.3   & 6676.3   & 6984.0\\
Humanoid-v4        & 7064.5   & 7228.4   & 6582.8   & 7316.1   & 6728.0   & 6984.0 \\
HumanoidStandup-v4 & 160131.6 & 160432.5 & 146507.5 & 161213.4 & 157304.5 & 157118.0\\
\bottomrule
\end{tabular}
\end{table}

\subsection{HIT Generation}
A human intelligence task (HIT) is a task posted on crowdsourcing platforms that needs answers. Each HIT consists of two sections: task description and queries. For Ant, Humanoid, and HumanoidStandup, task descriptions are adapted from descriptions available at the Gymnasium library and translated into Japanese. Robotics terminologies are rephrased with simpler terms and some details are removed. For example, "bipedal robot" is rephrased as "robot". Moreover, as an attempt for aligning crowdsourced anwsers with the groundtruth reward function, task descriptions are augmented with descriptions for the groundtruth reward function. For example, if the agent is penalized for too large control forces, then crowdworkers will be instructed not to prefer trajectories that contains sharp movements. Lastly, descriptions are also augmented with three to four examples, which consist of a query, an answer provided by the authors, and explanations for such answers. 
% Screenshots

A query consists of two trajectories to be compared and asks a crowdworker to select one from "A is better than B.", "A is similar to B.", and "A is worse than B". To improve the quality of crowdsourced answers, in each HIT queries are mixed with four trap questions~\citep{10.1145/1835449.1835542} whose answers can be effortlessly determined. Two of them are comparing a trajectory with itself. One is taken from the task description but with the order of trajectories switched. The other one is a easy question if the crowdworker reads the task descriptions. Crowdworkers are informed with the existence of trap questions and failing to answer them correctly leads to rejection of their answers for the HIT. As a post-processing step, answers to a HIT will be filtered out if any answer to trap questions is in correct.


